UntrustVul: An Automated Approach for Identifying Untrustworthy Alerts in Vulnerability Detection Models

Machine learning (ML) has shown promise in vulnerability detection, but ML detectors may rely on irrelevant code features, causing them to highlight non-vulnerable lines as suspicious. Such misleading predictions increase developers' manual effort and may lead to incorrect patching strategies, motivating the need to identify untrustworthy predictions automatically. We present UntrustVul, an approach for detecting untrustworthy vulnerability predictions by identifying suspicious lines that are inherently unrelated to vulnerabilities. UntrustVul leverages patterns from historical vulnerable lines and flags predictions as untrustworthy when the highlighted lines neither match known vulnerability patterns nor influence lines that do. A line is considered vulnerability-irrelevant if it does not resemble historical vulnerabilities and all its successors in the data and control dependency graph are also vulnerability-irrelevant. The approach is designed conservatively to minimise misclassifying trustworthy predictions as untrustworthy. We evaluate UntrustVul on 115K predictions from four models across the BigVul, MegaVul, SARD, and PrimeVul datasets. Results show that UntrustVul achieves AUC scores of 70%-88% and F1-scores of 82%-94%, outperforming existing approaches by 6%-59% in AUC and 13%-92% in F1-score.

==> sections/def_truthfulness.tex <==
Truthfulness is a complex concept, making it challenging for researchers to reach a consensus on an unified definition~\cite{Chander:2025:TowardTrustworthyArtificialIntelligenceTAIintheContextofExplainabilityandRobustness, Qu:2022:CombiningHumanandMachineConfidenceinTruthfulnessAssessment, Huang:2024:TrustLLM:TrustworthinessinLargeLanguageModels}. 
Although it is not easy to choose one specific definition, we consider truthfulness as the accurate representation of information, facts, and results~\cite{Huang:2024:TrustLLM:TrustworthinessinLargeLanguageModels}.
% Fulfilling condition (a) primarily depends on the system, whereas condition (b) involves the stakeholder.
% This definition is intentionally vague to emphasise its generalisability, making it challenging to quantify trustworthiness.
% Hence, we refine the definition for the context of vulnerability detection.
% For condition (a), a vulnerability detection model should correctly detect vulnerable code.
% For condition (b), with developers as the stakeholders, the model's decision-making should be plausible, meaning it is based on the actual root causes of vulnerabilities.
In the context of vulnerability detection, ML models make function-level predictions, which are either vulnerable or non-vulnerable, and the corresponding fine-grained interpretations. 
We refer to \textit{vulnerability predictions}, or shortly \textit{predictions}, as classifications that label code as vulnerable.
Accordingly, we define a \textit{truthful vulnerability prediction} as follows.
\begin{dfn} 
\label{def:trustworthy}
A truthful vulnerability prediction is correct, with its interpretation 
highlighting
% showing that it is based on 
vulnerability-triggering lines of code and their dependent lines.
\end{dfn}
% Assessing the trustworthiness of AI systems often requires the inspection of their behaviors and decision-making, i.e., by reviewing their explanations~\cite{Qinghua:2022:TowardsARoadmapOnSoftwareEngineeringForResponsibleAI}.
% Vulnerability detection models classify code as vulnerable or not.
% Prior studies~\cite{Ganz:2021:ExplainingGraphNeuralNetworksforVulnerabilityDiscovery, Chakraborty:2022:DeepLearningBasedVulnerabilityDetectionAreWeThereYet, Cheng:2024:BeyondFidelityExplainingVulnerabilityLocalizationofLearningBasedDetectors} have shown that while these predictions correctly detect vulnerable code, they may rely on irrelevant code features.
% Therefore, this paper examines the trustworthiness of vulnerability predictions, particularly whether they are based on the actual root causes.
\noindent
Following Definition~\ref{def:trustworthy}, a vulnerability prediction that heavily relies on irrelevant code features, e.g., identifiers, comments, and delimiters, is considered untruthful.
In this paper, we focus on correct vulnerability predictions only, as analysing the interpretations behind incorrect ones may be meaningless.

Truthfulness has been identified as a critical dimension of trustworthiness~\cite{Huang:2024:TrustLLM:TrustworthinessinLargeLanguageModels}. 
To assess trustworthiness as well as truthfulness, existing studies~\cite{Qinghua:2022:TowardsARoadmapOnSoftwareEngineeringForResponsibleAI, Chander:2025:TowardTrustworthyArtificialIntelligenceTAIintheContextofExplainabilityandRobustness, Cheng:2024:BeyondFidelityExplainingVulnerabilityLocalizationofLearningBasedDetectors} have acknowledged the use of ML explanations for 
% truthfulness assessment by 
disclosing the decision-making process.
% , thereby building human trust in ML systems.
These explanations are categorised as global~\cite{Caruana:2015:IntelligibleModelsforHealthCare:PredictingPneumoniaRiskandHospital30dayReadmission}, which provide insights into the entire model’s workings, and local~\cite{Ying:2019:GNNExplainer:GeneratingExplanationsforGraphNeuralNetworks, Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier, Li:2017:UnderstandingNeuralNetworksthroughRepresentationErasure}, which focuses on individual predictions. 
Local explanations, which break down a model into its components, allow users to grasp its decision-making process in a way that aligns with human cognitive patterns.
Hence, prior studies~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction, Ying:2019:GNNExplainer:GeneratingExplanationsforGraphNeuralNetworks} have leveraged them for fine-grained interpretations of vulnerability predictions at the line level.
% For example, LineVul~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction} applies the attention mechanism, while IVDetect~\cite{Li:2021:VulnerabilityDetectionwithFineGrainedInterpretations} uses GNNExplainer~\cite{Ying:2019:GNNExplainer:GeneratingExplanationsforGraphNeuralNetworks}.
% we leverage local explanations to uncover the reasoning behind individual predictions by highlighting the most relevant contributing features.
% Similarly, we leverage local explanations to uncover the reasoning behind vulnerability predictions for trustworthiness assessment.
Such interpretations, or explanations, take the form of a list of critical lines of code, each paired with an \textit{importance score} quantifying its contribution to the predictions.
Truthfulness of a vulnerability prediction then can be assessed by the alignment between its fine-grained interpretation
% , which often refers to its explanation,
and the actual vulnerabilities.

\lam{I plan to remove this paragraph.
Definition~\ref{def:trustworthy} describes a trustworthy vulnerability prediction, referring to local trustworthiness. 
In contrast, global trustworthiness is the ability to make trustworthy predictions across a broad range of inputs,
akin to domain experts.
% A globally trustworthy model can perfectly interpret every input like human domain experts.
Although global trustworthiness is the ultimate goal, it is challenging due to the complex architectures and training procedures required.
% , which result in higher computational costs. 
Hence, we focus on local trustworthiness of individual vulnerability predictions. 
While most observed vulnerability predictions by a model are trustworthy, this does not directly mean the entire model is trustworthy.}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/TrueVul (2).pdf}
%     % \vspace{-0.64cm}
%     \caption{The process of \truevul.}
%     \label{fig:truevul}
% \end{figure*}

==> sections/old_rq1.tex <==
\subsubsection*{\textbf{RQ1}: Relation between prediction uncertainty and trustworthiness}

We use model confidence as a metric to assess the uncertainty of vulnerability predictions. 
Figure~\ref{fig:correlation_trust_conf} illustrates the distribution of model confidence across two trustworthiness labels in the dataset of vulnerability predictions shown in Table~\ref{table:models_under_test}.
In all four models under test, most vulnerability predictions are untrustworthy.

For transformer-based models, the majority of vulnerability predictions have high confidence.
% The majority of high confidence predictions are untrustworthy. 
Among highly confident (0.9--1.0) predictions, untrustworthy predictions account for 75.4\%--86.5\%. 
Similarly, untrustworthy predictions with high confidence (0.8--0.9) represent 28.6\%--84.4\% of high-confidence predictions. 
On the other hand, confident (0.8--1.0) predictions can still be trustworthy, with 13.6\%--21.7\% of them being trustworthy. 
Predictions with low confidence ($<0.8$) can also be untrustworthy, making up 30.8\%--85.0\% of low-confidence predictions.

For GNN-based models, the distribution of model confidence contrasts with transformer-based models, with more low-confidence predictions and fewer high-confidence ones.
However, similarly to transformer-based models, most confident (0.8--1.0) predictions are untrustworthy, accounting for 98.8\%--99.2\%.
The majority of low-confidence ($<0.8$) are also untrustworthy, making up 95.0\%--95.7\% of low-confidence predictions.
In contrast, high- and low-confidence predictions can still be trustworthy, with 4.3\%--5.0\% of low-confidence predictions and 0.8\%--1.2\% of high-confidence predictions being untrustworthy.

It is clear that there is no significant relation between model confidence and trustworthiness.
For transformer-based models, the numbers of trustworthy and untrustworthy predictions both increase accordingly with higher confidence, whereas for graph-based models, they both decrease.
% The models are more likely to make confident predictions, while most of them are untrustworthy.

\begin{figure*}
    \centering
    \begin{minipage}{.324\linewidth}
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/linevul-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{LineVul~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/svuld-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{SVulD~\cite{Ni:2023:DistinguishingLookAlikeInnocentandVulnerableCodebySubtleSemanticRepresentationLearningandExplanation}}
        \end{subfigure}
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/ivdetect-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{IVDetect~\cite{Li:2021:VulnerabilityDetectionwithFineGrainedInterpretations}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/reveal-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{ReVeal~\cite{Chakraborty:2022:DeepLearningBasedVulnerabilityDetectionAreWeThereYet}}
        \end{subfigure}
        \caption{BigVul dataset}
    \end{minipage}
    \hfill
    \begin{minipage}{.324\linewidth}
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/linevul-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{LineVul~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/svuld-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{SVulD~\cite{Ni:2023:DistinguishingLookAlikeInnocentandVulnerableCodebySubtleSemanticRepresentationLearningandExplanation}}
        \end{subfigure}
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/ivdetect-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{IVDetect~\cite{Li:2021:VulnerabilityDetectionwithFineGrainedInterpretations}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/reveal-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{ReVeal~\cite{Chakraborty:2022:DeepLearningBasedVulnerabilityDetectionAreWeThereYet}}
        \end{subfigure}
        \caption{MegaVul dataset}
    \end{minipage}
    \hfill
    \begin{minipage}{.324\linewidth}
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/linevul-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{LineVul~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/svuld-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{SVulD~\cite{Ni:2023:DistinguishingLookAlikeInnocentandVulnerableCodebySubtleSemanticRepresentationLearningandExplanation}}
        \end{subfigure}
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/ivdetect-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{IVDetect~\cite{Li:2021:VulnerabilityDetectionwithFineGrainedInterpretations}}
        \end{subfigure}%
        \hfill
        \begin{subfigure}[ht]{0.49\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/reveal-rq1-hm_woi.pdf}
            \vspace{-5mm}
            \caption{ReVeal~\cite{Chakraborty:2022:DeepLearningBasedVulnerabilityDetectionAreWeThereYet}}
        \end{subfigure}
        \caption{SARD dataset}
    \end{minipage}
\end{figure*}

\begin{figure}[t]
    \centering
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/linevul-rq1-hm_woi.pdf}
        \vspace{-5mm}
        \caption{LineVul~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/svuld-rq1-hm_woi.pdf}
        \vspace{-5mm}
        \caption{SVulD~\cite{Ni:2023:DistinguishingLookAlikeInnocentandVulnerableCodebySubtleSemanticRepresentationLearningandExplanation}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/ivdetect-rq1-hm_woi.pdf}
        \vspace{-5mm}
        \caption{IVDetect~\cite{Li:2021:VulnerabilityDetectionwithFineGrainedInterpretations}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/reveal-rq1-hm_woi.pdf}
        \vspace{-5mm}
        \caption{ReVeal~\cite{Chakraborty:2022:DeepLearningBasedVulnerabilityDetectionAreWeThereYet}}
    \end{subfigure}
    % \vspace{-1mm}
    \caption{The distribution of predictions' confidence across trustworthiness labels.}
    \label{fig:correlation_trust_conf}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{minipage}{\linewidth}
    \centering
        \includegraphics[width=0.65\textwidth, clip, trim=2mm 2mm 1mm 2mm]{figures/chart_roc_note.pdf} 
        \vspace{2mm}
    \end{minipage}
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/chart_roc_tconf_linevul.pdf}
        \vspace{-5mm}
        \caption{LineVul~\cite{Fu:2022:LineVul:ATransformerBasedLineLevelVulnerabilityPrediction}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 2mm]{figures/chart_roc_tconf_svuld.pdf}
        \vspace{-5mm}
        \caption{SVulD~\cite{Ni:2023:DistinguishingLookAlikeInnocentandVulnerableCodebySubtleSemanticRepresentationLearningandExplanation}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/chart_roc_tconf_ivdetect.pdf}
        \vspace{-5mm}
        \caption{IVDetect~\cite{Li:2021:VulnerabilityDetectionwithFineGrainedInterpretations}}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth, clip, trim=1mm 2mm 1mm 0mm]{figures/chart_roc_tconf_reveal.pdf}
        \vspace{-5mm}
        \caption{ReVeal~\cite{Chakraborty:2022:DeepLearningBasedVulnerabilityDetectionAreWeThereYet}}
    \end{subfigure}
    % \vspace{-1mm}
    \caption{Comparing ROC curves between Naive and \truevul{}.}
    \label{fig:roc_curve}
\end{figure}

We further investigate the ability of model confidence to distinguish between trustworthy and untrustworthy predictions.
We consider a naive approach using model confidence to evaluate the trustworthiness of vulnerability predictions.
A vulnerability prediction is considered untrustworthy if its confidence is below the threshold $\theta_\text{\textit{conf}}$.
Figure~\ref{fig:correlation_trust_conf} shows that increasing $\theta_\text{\textit{conf}}$ on the y-axis increases the true positive rate, where untrustworthy predictions are correctly labeled, but also decreases the true negative rate, where trustworthy predictions are correctly labeled. 
In other words, increasing $\theta_\text{\textit{conf}}$ enhances Sensitivity but reduces Specificity.
We also plot ROC curves of the trustworthiness evaluation using model confidence, as shown in Figure~\ref{fig:roc_curve}.
The ROC curves across the models under test are near the random line.
Specifically, except for the ROC curve of SVulD,
% is above the random line, 
the ROC curves of other models fall below the random line.
This indicates model confidence is limited in distinguishing between trustworthy and untrustworthy predictions. 

\begin{custombox}[Answer to RQ1]
Uncertainty metrics of vulnerability predictions, such as model confidence, are not suitable for assessing their trustworthiness. 
 While most vulnerability predictions are untrustworthy, the numbers of trustworthy and untrustworthy predictions both increase or decrease accordingly as the threshold of prediction uncertainty changes.
% \aldeida{the second sentence could be written a bit more clearly. not clear what is meant by following similar trends}
% \lam{I revised that sentence.}
As a result, relying on these metrics easily overlooks trustworthy low-confidence predictions and untrustworthy high-confidence predictions, limiting their effectiveness in evaluating prediction trustworthiness.
\end{custombox}

==> tables/ablation.tex <==
% \begin{table*}[t]
% \caption{Comparing \truevul{} and its ablation variants, including one employing only line-level checking, and three without ensemble learning that use individual pre-trained models CodeBERT, GraphCodeBERT, and UniXcoder, respectively. The signs ``+'', ``-'', and ``='' indicate increases, decreases, and no changes in the effectiveness of \truevul{} compared to the ablation variants}
% \label{table:expr_ablation_results}
% \centering
% \setlength\tabcolsep{0pt} % default value: 6pt
% \resizebox{0.98\linewidth}{!}{%
% \begin{tabular}{c@{\hskip 2.5pt}|@{\hskip 2.5pt}l@{\hskip 2.5pt}|DDDDDDD|DDDDDDD|DDDDDDD}
% \toprule
% & \multicolumn{1}{c|}{\multirow{2}{*}{Variant}} & \multicolumn{7}{c|}{BigVul}                            & \multicolumn{7}{c|}{MegaVul} & \multicolumn{7}{c}{SARD} \\
% & \multicolumn{1}{c|}{}                         & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm   & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm  \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{LineVul\hspace{1.2mm}}}} 
% & Line-level only                              
% & +0.27 & +0.30 & +0.08 & +0.29 & +0.23 & +0.25 & +0.26 
% & +0.13 & +0.27 & +0.02 & +0.13 & +0.09 & +0.22 & +0.18
% & +0.42 & +0.37 & =     & +0.46 & +0.37 & =     & +0.31 \\
% & CodeBERT                                     
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     
% & -0.08 & +0.02 & -0.01 & -0.09 & -0.05 & +0.11 & +0.03
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     \\
% & GraphCodeBERT                                
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 
% & -0.09 & +0.05 & +0.01 & -0.10 & -0.06 & +0.11 & +0.02               
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 \\
% & UniXcoder                                    
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01 
% & +0.13 & +0.02 & =     & +0.15 & +0.09 & -0.10 & +0.03 
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01 \\               
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{SVulD\hspace{1.8mm}}}} 
% & Line-level only                              
% & +0.26 & +0.42 & +0.21 & +0.18 & +0.19 & +0.62 & +0.42 
% & +0.13 & +0.23 & +0.03 & +0.12 & +0.09 & +0.22 & +0.18 
% & -0.08 & +0.29 & +0.03 & -0.12 & -0.13 & +0.76 & +0.38 \\
% & CodeBERT                           
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & =     & +0.01    
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =    
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     \\
% & GraphCodeBERT                                
% & +0.02 & +0.02 & =     & +0.03 & +0.02 & =     & +0.02 
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01                
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 \\
% & UniXcoder                                    
% & =     & +0.01 & =     & =     & =     & +0.02 & +0.01 
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01                
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01 \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IVDetect\hspace{1mm}}}} 
% & Line-level only
% & +0.15 & +0.18 & +0.01 & +0.15 & +0.10 & +0.18 & +0.17 
% & +0.32 & +0.24 & +0.01 & +0.32 & +0.24 & +0.05 & +0.19 
% & +0.27 & +0.13 & =     & +0.28 & +0.19 & -0.11 & +0.09 \\
% & CodeBERT       
% & +0.01 & +0.01 & =     & +0.01 & +0.01 & =     & = 
% & =     & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     \\
% & GraphCodeBERT  
% & +0.01 & +0.01 & = & +0.01 & +0.01     & +0.03 & +0.02 
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 \\
% & UniXcoder      
% & +0.01 & =     & =     & +0.01 & =     & +0.01 & +0.01 
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01 
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01 \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ReVeal\hspace{1.8mm}}}} 
% & Line-level only
% & +0.24 & +0.14 & +0.01 & +0.25 & +0.17 & +0.01 & +0.13 
% & +0.24 & +0.24 & +0.01 & +0.25 & +0.19 & +0.09 & +0.17 
% & +0.29 & +0.14 & =     & +0.30 & +0.23 & -0.15 & +0.09 \\
% & CodeBERT       
% & +0.01 & =     & =     & +0.01 & =     & +0.01 & +0.01 
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     
% & +0.01 & +0.03 & =     & +0.01 & +0.01 & -0.01 & =     \\
% & GraphCodeBERT  
% & +0.01 & =     & =     & +0.01 & +0.01 & -0.01 & = 
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 
% & +0.01 & =     & +0.01 & +0.01 & =     & =     & +0.01 \\
% & UniXcoder      
% & +0.03 & =     & =     & +0.03 & +0.02 & +0.01 & +0.02 
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01
% & =     & +0.01 & =     & =     & =     & +0.01 & +0.01 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[t]
% \caption{Comparing \truevul{} with its ablation variants. 
% % We include one using only line-level checking and three without ensemble learning, each relying on a single pre-trained model: CodeBERT, GraphCodeBERT, or UniXcoder. 
% % ``Line-level only'' reflects the effectiveness of the variant using only line-level checking, while 
% ``Single-model only'' represents the average effectiveness of three single-model variants. 
% Symbols ``+'', ``-'', and ``='' indicate increases, decreases, and no changes compared to \truevul}
% \label{table:expr_ablation_results}
% \centering
% \setlength\tabcolsep{0pt} % default value: 6pt
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l@{\hskip 2.5pt}|@{\hskip 2.5pt}l@{\hskip 2.5pt}|CCCCCCC|CCCCCCC|CCCCCCC}
% \toprule
% & \multicolumn{1}{c|}{\multirow{2}{*}{Variant}} & \multicolumn{7}{c|}{BigVul}                            & \multicolumn{7}{c|}{MegaVul} & \multicolumn{7}{c}{SARD} \\
% & \multicolumn{1}{c|}{}                         & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm   & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm  \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{LineVul\hspace{-0.5mm}}}} 
% & Line-level only                              
% & 0.51 & 0.56 & 0.89 & 0.48 & 0.63 & 0.58 & 0.54 
% & 0.70 & 0.61 & 0.97 & 0.71 & 0.81 & 0.54 & 0.62
% & 0.42 & 0.47 & 1.00 & 0.37 & 0.54 & 1.00 & 0.60 \\
% & Dependency-level only                                     
% & 0.73 & 0.76 & 0.94 & 0.73 & 0.82 & 0.72 & 0.72     
% & 0.80 & 0.80 & 0.98 & 0.83 & 0.89 & 0.68 & 0.76
% & 0.89 & 0.70 & 0.97 & 0.90 & 0.94 & 0.75 & 0.82 \\
% & Single-model only                                     
% & 0.77 & 0.84 & 0.97    & 0.76 & 0.86     & 0.83     & 0.79     
% & 0.84 & 0.85 & 0.99     & 0.85 & 0.91 & 0.72 & 0.77
% & 0.83 & 0.83 & 1.00     & 0.84 & 0.91     & 1.00     & 0.90 \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{SVulD\hspace{-0.5mm}}}} 
% & Line-level only                              
% & +0.26 & +0.42 & +0.21 & +0.18 & +0.19 & +0.62 & +0.42 
% & +0.13 & +0.23 & +0.03 & +0.12 & +0.09 & +0.22 & +0.18 
% & -0.08 & +0.29 & +0.03 & -0.12 & -0.13 & +0.76 & +0.38 \\
% & Dependency-level only                                     
% & +0.13 & +0.20 & -0.03 & +0.10 & +0.06 & +0.32 & +0.20     
% & +0.03 & +0.06 & +0.01 & +0.03 & +0.01 & +0.08 & +0.06
% & +0.11 & +0.18 & +0.03 & -0.01 & -0.01 & +0.51 & +0.25 \\
% & Single-model only                           
% & +0.01 & +0.02 & =     & +0.01 & +0.01 & +0.01 & +0.01    
% & +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01    
% & +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01 \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IVDetect\hspace{-0.5mm}}}} 
% & Line-level only
% & +0.15 & +0.18 & +0.01 & +0.15 & +0.10 & +0.18 & +0.17 
% & +0.32 & +0.24 & +0.01 & +0.32 & +0.24 & +0.05 & +0.19 
% & +0.27 & +0.13 & =     & +0.28 & +0.19 & -0.11 & +0.09 \\
% & Dependency-level only                                     
% & +0.16 & +0.21 & =     & +0.17 & +0.10 & +0.16 & +0.16     
% & +0.06 & +0.06 & =     & +0.06 & +0.04 & +0.13 & +0.10
% & +0.13 & +0.16 & +0.01 & +0.13 & +0.08 & +0.05 & +0.08 \\
% & Single-model only       
% & +0.01 & +0.01 & =     & +0.01 & +0.01 & +0.01 & +0.01 
% & =     & +0.01 & =     & +0.01 & =     & =     & +0.01     
% & +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01 \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ReVeal\hspace{-0.5mm}}}} 
% & Line-level only
% & +0.24 & +0.14 & +0.01 & +0.25 & +0.17 & +0.01 & +0.13 
% & +0.24 & +0.24 & +0.01 & +0.25 & +0.19 & +0.09 & +0.17 
% & +0.29 & +0.14 & =     & +0.30 & +0.23 & -0.15 & +0.09 \\
% & Dependency-level only                                     
% & +0.17 & +0.16 & =     & +0.18 & +0.11 & +0.09 & +0.13     
% & +0.03 & +0.03 & =     & +0.03 & +0.03 & +0.04 & +0.04
% & +0.14 & +0.07 & +0.01 & +0.14 & +0.09 & -0.01 & +0.06 \\
% & Single-model only       
% & +0.02 & =     & =     & +0.02 & +0.01 & =     & +0.01 
% & +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01     
% & +0.01 & +0.02 & =     & +0.01 & =     & =     & +0.01 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


\begin{table*}[t]
\caption{Comparing \truevul{} with its ablation variants. 
% We include one using only line-level checking and three without ensemble learning, each relying on a single pre-trained model: CodeBERT, GraphCodeBERT, or UniXcoder. 
% ``Line-level only'' reflects the effectiveness of the variant using only line-level checking, while 
``Single-model only'' represents the average effectiveness of three single-model variants. 
Symbols ``+'', ``-'', and ``='' indicate increases, decreases, and no changes compared to \truevul}
\label{table:expr_ablation_results}
\centering
\setlength\tabcolsep{0pt} % default value: 6pt
\resizebox{\linewidth}{!}{%
\begin{tabular}{|@{\hspace{2pt}}l@{\hskip 2.5pt}|@{\hskip 2.5pt}l@{\hskip 2.5pt}|DDDDDDD|DDDDDDD|DDDDDDD|}
\hline
& \multicolumn{1}{c|}{\multirow{2}{*}{Variant}} & \multicolumn{7}{c|}{BigVul}                            & \multicolumn{7}{c|}{MegaVul} & \multicolumn{7}{c|}{SARD} \\
& \multicolumn{1}{c|}{}                         & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm   & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm & $\Delta$Acc  & $\Delta$Auc  & $\Delta$Pre  & $\Delta$Sen  & $\Delta$F1   & $\Delta$Spe  & $\Delta$Gm  \\
\hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{LineVul}}} 
& Line-level only                              
& +0.27 & +0.30 & +0.08 & +0.29 & +0.23 & +0.25 & +0.26 
& +0.13 & +0.27 & +0.02 & +0.13 & +0.09 & +0.22 & +0.18
& +0.42 & +0.37 & =     & +0.46 & +0.37 & =     & +0.31 \\
& Dependency-level only                                     
& +0.05 & +0.10 & +0.03 & +0.04 & +0.04 & +0.11 & +0.08     
& +0.03 & +0.08 & +0.01 & +0.01 & +0.01 & +0.08 & +0.04
& -0.05 & +0.14 & +0.03 & -0.07 & -0.03 & +0.25 & +0.09 \\
& Single-model only                                     
& +0.01 & +0.02 & =     & +0.01 & =     & =     & +0.01     
& -0.01 & +0.03 & =     & -0.01 & -0.01 & +0.04 & +0.03
& +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01 \\
\hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{SVulD}}} 
& Line-level only                              
& +0.26 & +0.42 & +0.21 & +0.18 & +0.19 & +0.62 & +0.42 
& +0.13 & +0.23 & +0.03 & +0.12 & +0.09 & +0.22 & +0.18 
& -0.08 & +0.29 & +0.03 & -0.12 & -0.13 & +0.76 & +0.38 \\
& Dependency-level only                                     
& +0.13 & +0.20 & -0.03 & +0.10 & +0.06 & +0.32 & +0.20     
& +0.03 & +0.06 & +0.01 & +0.03 & +0.01 & +0.08 & +0.06
& +0.11 & +0.18 & +0.03 & -0.01 & -0.01 & +0.51 & +0.25 \\
& Single-model only                           
& +0.01 & +0.02 & =     & +0.01 & +0.01 & +0.01 & +0.01    
& +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01    
& +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01 \\
\hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{IVDetect}}} 
& Line-level only
& +0.15 & +0.18 & +0.01 & +0.15 & +0.10 & +0.18 & +0.17 
& +0.32 & +0.24 & +0.01 & +0.32 & +0.24 & +0.05 & +0.19 
& +0.27 & +0.13 & =     & +0.28 & +0.19 & -0.11 & +0.09 \\
& Dependency-level only                                     
& +0.16 & +0.21 & =     & +0.17 & +0.10 & +0.16 & +0.16     
& +0.06 & +0.06 & =     & +0.06 & +0.04 & +0.13 & +0.10
& +0.13 & +0.16 & +0.01 & +0.13 & +0.08 & +0.05 & +0.08 \\
& Single-model only       
& +0.01 & +0.01 & =     & +0.01 & +0.01 & +0.01 & +0.01 
& =     & +0.01 & =     & +0.01 & =     & =     & +0.01     
& +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01 \\
\hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ReVeal}}} 
& Line-level only
& +0.24 & +0.14 & +0.01 & +0.25 & +0.17 & +0.01 & +0.13 
& +0.24 & +0.24 & +0.01 & +0.25 & +0.19 & +0.09 & +0.17 
& +0.29 & +0.14 & =     & +0.30 & +0.23 & -0.15 & +0.09 \\
& Dependency-level only                                     
& +0.17 & +0.16 & =     & +0.18 & +0.11 & +0.09 & +0.13     
& +0.03 & +0.03 & =     & +0.03 & +0.03 & +0.04 & +0.04
& +0.14 & +0.07 & +0.01 & +0.14 & +0.09 & -0.01 & +0.06 \\
& Single-model only       
& +0.02 & =     & =     & +0.02 & +0.01 & =     & +0.01 
& +0.01 & +0.01 & =     & +0.01 & =     & =     & +0.01     
& +0.01 & +0.02 & =     & +0.01 & =     & =     & +0.01 \\
\hline
\end{tabular}%
}
\end{table*}


==> tables/effectiveness_cr_sim.tex <==
\begin{table*}
\centering
\caption{The \textit{cross-project} effectiveness of \truevul{} (ours) and the baselines on MegaVul, SARD, and PrimeVul}
\label{table:expr_results_cp}
\vspace{-3mm}
\setlength\tabcolsep{2.5pt} % default value: 6pt

\subfloat[LineVul - MegaVul]{%
\begin{tabular}{|l|CCCC|}
\hline
             & Acc  & Auc   & F1   & Gm  \\
\hline
\truevul     & 0.83 & 0.88 & 0.90 & 0.80 \\
Naive        & 0.25 & 0.34 & 0.39 & 0.37 \\
PerturbVar   & 0.14 & 0.32 & 0.23 & 0.30 \\
PerturbAPI   & 0.04 & 0.67 & 0.05 & 0.14 \\
PerturbJoint & 0.13 & 0.67 & 0.21 & 0.29 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[SVulD - MegaVul]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc  & F1   & Gm  \\
\hline
0.82 & 0.82 & 0.89 & 0.79 \\
0.47 & 0.46 & 0.62 & 0.48 \\
0.33 & 0.52 & 0.48 & 0.46 \\
0.29 & 0.51 & 0.43 & 0.45 \\
0.34 & 0.51 & 0.49 & 0.47 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[IVDetect - MegaVul]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc  & F1   & Gm   \\
\hline
0.81 & 0.74 & 0.89 & 0.75 \\
0.22 & 0.30 & 0.35 & 0.36 \\
0.03 & 0.30 & 0.02 & 0.09 \\
0.02 & 0.32 & 0.01 & 0.08 \\
0.03 & 0.32 & 0.03 & 0.12 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[ReVeal - MegaVul]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc  & F1   & Gm   \\
\hline
0.72 & 0.70 & 0.84 & 0.68 \\
0.37 & 0.36 & 0.54 & 0.41 \\
0.02 & 0.32 & 0.01 & 0.09 \\
0.02 & 0.37 & 0.01 & 0.08 \\
0.03 & 0.35 & 0.01 & 0.10 \\
\hline
\end{tabular}%
}

\subfloat[LineVul - SARD]{%
\begin{tabular}{|l|CCCC|}
\hline
             & Acc  & Auc   & F1   & Gm   \\
\hline
\truevul     & 0.84 & 0.84  & 0.91 & 0.91 \\
Naive        & 0.80 & 0.76  & 0.88 & 0.78 \\
PerturbVar   & 0.36 & 0.78  & 0.45 & 0.54 \\
PerturbAPI   & 0.24 & 0.91  & 0.29 & 0.42 \\
PerturbJoint & 0.27 & 0.86  & 0.33 & 0.44 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[SVulD - SARD]{%
\begin{tabular}{|CCCC|}
\hline
Acc     & Auc     & F1   & Gm   \\
\hline
0.76    & 0.82    & 0.78   & 0.78   \\
0.63    & 0.56    & 0.77    & 0.55   \\
0.13    & 0.56    & 0.18   &  0.3   \\
0.12    & 0.55    & 0.16   & 0.29   \\
0.14    & 0.55    & 0.21    & 0.32 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[IVDetect - SARD]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc & F1  & Gm   \\
\hline
0.85 & 0.82 & 0.92 & 0.76 \\
0.19 & 0.23 & 0.30 & 0.31 \\
0.04 & 0.23 & 0.02 & 0.10 \\
0.03 & 0.23 & 0.00 & 0.00 \\
0.04 & 0.24 & 0.02 & 0.09 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[ReVeal - SARD]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc   & F1   & Gm   \\
\hline
0.75 & 0.71 & 0.85 & 0.68 \\
0.23 & 0.28 & 0.35 & 0.33 \\
0.03     & 0.28     & 0.01     & 0.03     \\
0.03     & 0.29     & 0.00    & 0.00     \\
0.03     & 0.29     & 0.01  & 0.03     \\
\hline
\end{tabular}%
}

\subfloat[LineVul - PrimeVul]{%
\begin{tabular}{|l|CCCC|}
\hline
             & Acc  & Auc   & F1   & Gm   \\
\hline
\truevul & 0.78 & 0.82    & 0.87   & 0.79 \\
Naive        & 0.53    & 0.57    & 0.66    & 0.54   \\
PerturbVar   & 0.19  &  0.55   & 0.18   & 0.30  \\
PerturbAPI   & 0.12 & 0.75    & 0.03   & 0.12 \\
PerturbJoint & 0.18 & 0.76    & 0.16   & 0.29  \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[SVulD - PrimeVul]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc   & F1   & Gm   \\
\hline
0.83    & 0.88     & 0.90   & 0.86   \\
0.60    & 0.60    & 0.74     & 0.57   \\
0.25  &  0.57   & 0.34     & 0.42  \\
0.20 & 0.56     & 0.26   & 0.36 \\
0.24 & 0.57    & 0.33     & 0.40  \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[IVDetect - PrimeVul]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc & F1   & Gm   \\
\hline
0.79 & 0.82 & 0.88 & 0.79 \\
0.50 & 0.31 & 0.67 & 0.37 \\
0.03 & 0.25 & 0.02 & 0.09 \\
0.03 & 0.32 & 0.01 & 0.00 \\
0.04 & 0.27 & 0.03 & 0.12 \\
\hline
\end{tabular}%
}
\hspace{1pt}
\subfloat[ReVeal - PrimeVul]{%
\begin{tabular}{|CCCC|}
\hline
Acc  & Auc   & F1   & Gm   \\
\hline
0.62 & 0.76 & 0.76 & 0.73 \\
0.53 & 0.33 & 0.69 & 0.38 \\
0.03     & 0.35     & 0.01     & 0.04     \\
0.03     & 0.35     & 0.01     & 0.06     \\
0.03     & 0.37     & 0.01     & 0.07     \\
\hline
\end{tabular}%
}


% \vspace{-5mm}
\end{table*}
